StyleDrop: Text-to-Image Generation in Any Style

Pre-trained large text-to-image models synthesize impressive images with an appropriate use of text prompts. However, ambiguities inherent in natural language and out-of-distribution effects make it hard to synthesize image styles, that leverage a specific design pattern, texture or material. In this paper, we introduce StyleDrop, a method that enables the synthesis of images that faithfully follow a specific style using a text-to-image model. The proposed method is extremely versatile and captures nuances and details of a user-provided style, such as color schemes, shading, design patterns, and local and global effects. It efficiently learns a new style by fine-tuning very few trainable parameters (less than $1\%$ of total model parameters) and improving the quality via iterative training with either human or automated feedback. Better yet, StyleDrop is able to deliver impressive results even when the user supplies only a single image that specifies the desired style. An extensive study shows that, for the task of style tuning text-to-image models, StyleDrop implemented on Muse convincingly outperforms other methods, including DreamBooth and textual inversion on Imagen or Stable Diffusion. More results are available at our project website: https://styledrop.github.io

==> figure/tex/supp_ablation_multi_concept.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figure/hq/my_asset_in_my_style.pdf}
    \caption{{\color{red}[[PLACEHOLDER for MULTI-CONCEPT JOINT TRAINING ABLATION]]}}
    \label{fig:supp_ablation_multi_concept}
\end{figure}
